Zeroth-Order Fine-Tuning of LLMs with Extreme Sparsity

Zeroth-order optimization (ZO) is a memory-efficient strategy for fine-tuning Large Language Models using only forward passes. However, the application of ZO fine-tuning in memory-constrained settings such as mobile phones and laptops is still challenging since full precision forward passes are infeasible. In this study, we address this limitation by integrating sparsity and quantization into ZO fine-tuning of LLMs. Specifically, we investigate the feasibility of fine-tuning an extremely small subset of LLM parameters using ZO. This approach allows the majority of un-tuned parameters to be quantized to accommodate the constraint of limited device memory. Our findings reveal that the pre-training process can identify a set of "sensitive parameters" that can guide the ZO fine-tuning of LLMs on downstream tasks. Our results demonstrate that fine-tuning 0.1% sensitive parameters in the LLM with ZO can outperform the full ZO fine-tuning performance, while offering wall-clock time speedup. Additionally, we show that ZO fine-tuning targeting these 0.1% sensitive parameters, combined with 4 bit quantization, enables efficient ZO fine-tuning of an Llama2-7B model on a GPU device with less than 8 GiB of memory and notably reduced latency.

==> tables/experiment_meta_data_ablation.tex <==
\begin{table}[!htbp]
     \setlength{\tabcolsep}{4pt}
     \renewcommand{\arraystretch}{1.15} % Default value: 1
     \fontsize{8pt}{8pt}\selectfont
    \centering

    \vspace{-1.3em}
    \caption{The chosen hyperparameters for experiments in Figure~\ref{fig:ablation-sensitive-weights-random} and Figure~\ref{fig:ablation-sensitive-static-dynamic}. We repeat each hyperparameters for 3 random trials and report the average to draw a line in Figure~\ref{fig:ablation-sensitive-weights-random} and Figure~\ref{fig:ablation-sensitive-static-dynamic}, and we use LlaMA2-7B for all experiments. For each subtable, we include the fraction to optimize on its header and report the chosen learning rate on each cell. } \label{tab:meta-data-ablation}

    \begin{subtable}[!ht]{\textwidth}
    \caption{\textbf{RTE}}
    \vspace{-0.5em}

    
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l ccccc r}
    \toprule    
     & \textbf{Methods} & 1e-5 & 1e-4 & 1e-3 & 1e-2 & 1e-1 \\ \hline
    
    \midrule

     & \textbf{Sensitive (C4, static)} ($\eps=$1e-3) & 1e-5 & 1e-6 & 1e-6 & 1e-6 & 1e-6 \\ 

     & \textbf{Sensitive (task-specific, static)} ($\eps=$1e-3) & 1e-5 & 1e-6 & 1e-6 & 1e-6 & 1e-6 \\ 

     & \textbf{Sensitive (task-specific, dynamic)} ($\eps=$1e-3) & 1e-5 & 1e-6 & 1e-6 & 1e-6 & 1e-6  \\ 

     & Random (static) ($\eps=$1e-3) & 2e-2 & 5e-3 & 5e-4 & 5e-5 & 5e-5 \\ 

     & Random (dynamic) ($\eps=$1e-3) & 2e-2 & 5e-3 & 2e-4 & 5e-5 & 5e-6 \\ 

     & Weight outliers (static) ($\eps=$1e-3) & 2e-3 & 1e-3 & 2e-4 & 5e-5 & 1e-5 \\ 

    \bottomrule 
    \end{tabular*}
    \end{subtable}


    \begin{subtable}[!ht]{\textwidth}
    \caption{\textbf{WiC}}
    \vspace{-0.5em}

    
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l ccccc r}
    \toprule    
     & \textbf{Methods} & 1e-5 & 1e-4 & 1e-3 & 1e-2 & 1e-1 \\ \hline
    
    \midrule

     & \textbf{Sensitive (C4, static)} ($\eps=$1e-3) & 1e-5 & 2e-6 & 1e-6 & 1e-6 & 1e-6 \\ 

     & \textbf{Sensitive (task-specific, static)} ($\eps=$1e-3) & 1e-5 & 2e-6 & 1e-6 & 1e-6 & 1e-6 \\ 

     & \textbf{Sensitive (task-specific, dynamic)} ($\eps=$1e-3) & 1e-5 & 2e-6 & 1e-6 & 1e-6 & 1e-6 \\ 

     & Random (static) ($\eps=$1e-3) & 2e-2 & 5e-3 & 5e-4 & 5e-5 & 5e-6 \\ 

     & Random (dynamic) ($\eps=$1e-3) & 2e-2 & 5e-3 & 5e-4 & 5e-5 & 5e-6 \\ 

     & Weight outliers (static) ($\eps=$1e-3) & 1e-3 & 5e-4 & 2e-4 & 1e-4 & 2e-5 \\ 

    \bottomrule 
    \end{tabular*}
    \end{subtable}


    \begin{subtable}[!ht]{\textwidth}
    \caption{\textbf{COPA}}
    \vspace{-0.5em}

    
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l ccccc r}
    \toprule    
     & \textbf{Methods} & 1e-5 & 1e-4 & 1e-3 & 1e-2 & 1e-1 \\ \hline
    
    \midrule

     & \textbf{Sensitive (C4, static)} ($\eps=$1e-3) & 5e-6 & 1e-6 & 1e-6 & 1e-6 & 5e-7 \\ 

     & \textbf{Sensitive (task-specific, static)} ($\eps=$1e-3) & 5e-6 & 2e-6 & 2e-6 & 1e-6 & 1e-6  \\ 

     & \textbf{Sensitive (task-specific, dynamic)} ($\eps=$1e-3) & 5e-6 & 1e-6 & 1e-6 & 1e-6 & 1e-6 \\ 

     & Random (static) ($\eps=$1e-3) & 1e-2 & 2e-3 & 5e-4 & 5e-5 & 5e-6 \\ 

     & Random (dynamic) ($\eps=$1e-3) & 2e-3 & 1e-3 & 2e-4 & 2e-5 & 2e-6 \\ 

     & Weight outliers (static) ($\eps=$1e-3) & 1e-3 & 5e-4 & 5e-4 & 1e-4 & 1e-5 \\ 

    \bottomrule 
    \end{tabular*}
    \end{subtable}


\end{table}

% 

==> tables/experiment_meta_data_main_results.tex <==
\begin{table}[!htbp]
     \setlength{\tabcolsep}{4pt}
     \renewcommand{\arraystretch}{1.15} % Default value: 1
     \fontsize{8pt}{8pt}\selectfont
    \centering

    \vspace{-1.3em}
    \caption{The chosen hyperparameters for experiments in Table~\ref{tab:main-results}. We repeat each hyperparameters for 3 random trials and report the average and standard deviation in Table~\ref{tab:main-results}.} \label{tab:meta-data-main-results}

    \begin{subtable}[!ht]{\textwidth}
    \caption{\textbf{LlaMA2-7B}}
    \vspace{-0.5em}

    
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l |c | cccccccr}
    \toprule    
     & \textbf{Methods} & SST-2 & RTE & CB & BoolQ & WSC & WiC & COPA \\ \hline
    
    \midrule

     Q, ZO & \textbf{Sensitive (C4, static)} ($\eps=$1e-3) & 5e-7 & 1e-6 & 1e-6 & 1e-6 & 5e-7 & 1e-6 & 1e-6  \\ 

     & LoRA ($\eps=$1e-3) & 1e-5 & 5e-5 & 1e-5 & 2e-5 & 1e-5 & 2e-5 & 1e-5 \\ 

     & Prefix ($\eps=$1e-2) & 1e-4 & 2e-4 & 5e-4 & 5e-4 & 1e-4 & 5e-4 & 2e-4  \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} ($\eps=$1e-3) & 5e-7 & 1e-6 & 1e-6 & 1e-6 & 1e-6 & 1e-6 & 2e-6 \\ 

     & Random (static) ($\eps=$1e-3) & 2e-4 & 5e-4 & 2e-4 & 5e-4 & 2e-4 & 5e-4 & 5e-4  \\ 

     & Full fine-tuning ($\eps=$1e-3) & 5e-7 & 5e-7 & 5e-7 & 5e-7 & 2e-7 & 5e-7 & 5e-7 \\ 

     \midrule

     & ICL (\#examples) & 16 & 16 & 16 & 8 & 16 & 8 & 8  \\ 
     

    \bottomrule 
    \end{tabular*}
    \end{subtable}



    \vspace{-0.5em}
    \begin{subtable}[!ht]{\textwidth}
    \caption{\textbf{Mistral-7B}}
    \vspace{-0.5em}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l |c | cccccccr}

    \midrule

    Q, ZO & \textbf{Sensitive (C4, static)} ($\eps=$1e-4) & 2e-8 & 5e-8 & 2e-8 & 2e-8 & 1e-8 & 2e-8 & 2e-8 \\ 

     & LoRA ($\eps=$1e-4) & 2e-6 & 5e-6 & 2e-6 & 2e-6 & 2e-6 & 2e-6 & 2e-6  \\ 

     & Prefix ($\eps=$1e-3) & 1e-3 & 2e-3 & 1e-3 & 1e-2 & 5e-4 & 1e-3 & 5e-4  \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} ($\eps=$1e-4) & 5e-8 & 5e-8 & 2e-8 & 2e-8 & 2e-8 & 2e-8 & 2e-8 \\ 

     & Random (static) ($\eps=$1e-4) & 1e-5 & 2e-6 & 5e-6 & 1e-5 & 1e-6 & 2e-6 & 2e-5 \\ 

     & Full fine-tuning ($\eps=$1e-4) & 2e-8 & 2e-8 & 1e-8 & 1e-8 & 1e-8 & 1e-8 & 2e-8  \\ 

     \midrule

     & ICL (\#examples) & 4 & 8 & 4 & 16 & 4 & 4 & 8  \\ 
    


    \bottomrule 
    \end{tabular*}    
    
    \end{subtable}


    \begin{subtable}[!ht]{\textwidth}
    \vspace{-0.5em}
    \caption{\textbf{OPT-6.7B}}
    \vspace{-0.5em}

    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l |c | cccccccr}

    \midrule

    Q, ZO & \textbf{Sensitive (C4, static)} ($\eps=$1e-3) & 2e-7 & 5e-7 & 5e-7 & 5e-7 & 2e-7 & 5e-7 & 2e-7 \\ 

     & LoRA ($\eps=$1e-3) & 1e-5 & 2e-5 & 1e-5 & 2e-5 & 1e-5 & 2e-5 & 2e-5 \\ 
     
     & Prefix ($\eps=$1e-2) & 2e-3 & 1e-2 & 1e-3 & 5e-3 & 5e-3 & 1e-2 & 5e-3 \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} ($\eps=$1e-3) & 2e-7 & 5e-7 & 5e-7 & 2e-7 & 2e-7 & 5e-7 & 2e-7 \\ 
     
     & Random (static) ($\eps=$1e-3) & 1e-4 & 5e-5 & 2e-5 & 5e-5 & 2e-4 & 5e-5 & 5e-5 \\ 

     & Full fine-tuning ($\eps=$1e-3) & 2e-7 & 2e-7 & 2e-7 & 2e-7 & 2e-7 & 2e-7 & 5e-7 \\ 

     \midrule

     & ICL (\#examples) & 16 & 4 & 16 & 16 & 16 & 8 & 16 \\ 
     

    \bottomrule 
    \end{tabular*}   

    \end{subtable}

\end{table}

% 

==> tables/llama2_7b.tex <==
\begin{table}[!htbp]
     \setlength{\tabcolsep}{3.8pt}
     \renewcommand{\arraystretch}{1.25} % Default value: 1
     {\fontsize{8pt}{8pt}\selectfont
    \centering

    
    \caption{Experiments on LLaMA2-7B. ``Q'' means the full model is quantized with 4-bit quantization method (SqueezeLLM~\citep{kim2023squeezellm}), and ``ZO'' means the model is finetuned with ZO-SGD optimizer. For each trial, we use the same hyperparameters and repeat it with 3 random seeds. We report the average and standard deviation of test set accuracy in the format of \textbf{\val{\text{mean}}{\text{std}}}.} \label{tab:llama2-7b}
    
    \begin{tabular}{l |c | ccccccc | ccr}
    \toprule    
     & \textbf{Methods} & SST-2 & RTE & CB & BoolQ & WSC & WiC & COPA & \textbf{Acc} & \textbf{Rank} \\ \hline
    
    \midrule

     Q, ZO & \textbf{Sensitive (C4, static)} & \val{\textbf{94.7}}{0.4} & \val{\textbf{74.7}}{1.2} & \val{\textbf{66.7}}{2.2} & \val{\textbf{83.0}}{0.5} & \val{57.4}{3.9} & \val{\textbf{65.2}}{0.9} & \val{85.0}{2.2} & \textbf{75.2} & \textbf{2.43} \\ 

     & LoRA & \val{93.8}{0.6} & \val{64.7}{1.1} & \val{64.9}{4.7} & \val{79.7}{1.1} & \val{\textbf{61.5}}{2.1} & \val{59.8}{0.1} & \val{\textbf{85.7}}{0.5} & 72.9 & 4.29 \\ 

     & Prefix & \val{80.5}{4.3} & \val{65.5}{1.2} & \val{63.1}{3.0} & \val{80.3}{0.2} & \val{54.5}{11.4} & \val{58.3}{1.3} & \val{82.0}{0.8} & 69.2 & 5.86 \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} & \val{\textbf{94.8}}{0.1} & \val{\textbf{73.6}}{0.9} & \val{\textbf{69.1}}{2.2} & \val{\textbf{83.5}}{0.8} & \val{57.4}{4.7} & \val{64.2}{1.1} & \val{\textbf{83.7}}{2.4} & \textbf{75.2} & \textbf{2.29} \\ 

     & Random (static) & \val{94.1}{0.3} & \val{68.0}{1.7} & \val{64.9}{3.4} & \val{77.0}{0.7} & \val{\textbf{59.6}}{3.6} & \val{\textbf{64.8}}{1.1} & \val{83.3}{1.7} & 73.1 & 4.14  \\ 

     & Full fine-tuning & \val{94.6}{0.5} & \val{73.3}{5.1} & \val{66.7}{0.8} & \val{81.9}{0.8} & \val{58.0}{4.3} & \val{61.9}{0.2} & \val{82.7}{1.7} & 74.2 & 3.57 \\ 

     \midrule

     & Zero-shot & \val{89.0}{0.0} & \val{57.8}{0.0} & \val{32.1}{0.0} & \val{69.9}{0.2} & \val{50.2}{0.0} & \val{36.5}{0.0} & \val{79.0}{0.0} & 59.2 & 7.29 \\ 


     & ICL & \val{94.8}{0.2} & \val{71.5}{4.3} & \val{72.6}{15.2} & \val{77.5}{4.6} & \val{53.2}{1.1} & \val{61.1}{4.3} & \val{87.0}{2.2} & 74.0 & 3.43 \\ 
     

    \bottomrule 
    \end{tabular}    
    }
\end{table}

% 

==> tables/mistral_7b.tex <==
\begin{table}[!htbp]
     \setlength{\tabcolsep}{3.8pt}
     \renewcommand{\arraystretch}{1.25} % Default value: 1
     \fontsize{8pt}{8pt}\selectfont
    \centering
    \label{tab:mistral-6.7b}
    \caption{Experiments on Mistral-7B. }
    
    \begin{tabular}{l |c | ccccccc | cc r}
    \toprule    
     & \textbf{Methods} & SST-2 & RTE & CB & BoolQ & WSC & WiC & COPA & \textbf{Acc} & \textbf{Rank} \\ \hline
    
    \midrule



    Q, ZO & \textbf{Sensitive (C4, static)} & \val{\textbf{94.0}}{0.3} & \val{\textbf{74.2}}{2.7} & \val{\textbf{70.2}}{2.2} & \val{\textbf{75.1}}{2.4} & \val{59.6}{4.9} & \val{\textbf{61.2}}{0.9} & \val{\textbf{88.3}}{1.2} & \textbf{74.7} & \textbf{2.86} \\ 

     & LoRA & \val{\textbf{94.0}}{0.4} & \val{65.3}{1.3} & \val{64.3}{1.5} & \val{70.3}{3.7} & \val{\textbf{60.9}}{3.7} & \val{61.1}{0.4} & \val{\textbf{88.3}}{0.5} & 72.0 & 3.57 \\ 

     & Prefix & \val{86.9}{2.1} & \val{57.3}{1.4} & \val{63.7}{5.9} & \val{62.2}{0.9} & \val{60.3}{4.6} & \val{49.0}{0.3} & \val{81.3}{1.7} & 65.8 & 4.86 \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} & \val{\textbf{94.7}}{0.3} & \val{\textbf{77.1}}{0.9} & \val{\textbf{69.0}}{0.8} & \val{\textbf{78.4}}{2.2} & \val{\textbf{58.0}}{4.3} & \val{61.4}{0.2} & \val{\textbf{89.3}}{1.3} & \textbf{75.4} & \textbf{1.86} \\ 

     & Random (static) & \val{87.9}{1.9} & \val{50.2}{0.8} & \val{66.1}{4.4} & \val{60.6}{1.7} & \val{57.6}{1.4} & \val{57.3}{0.8} & \val{81.3}{1.2} & 65.9 & 5.29 \\ 

     & Full fine-tuning & \val{94.6}{0.1} & \val{74.6}{2.1} & \val{68.8}{6.2} & \val{76.6}{0.2} & \val{54.8}{6.2} & \val{\textbf{62.6}}{0.5} & \val{88.3}{0.5} & 74.3 & 2.86  \\ 

     \midrule

    & Zero-shot & \val{54.8}{0.0} & \val{50.5}{0.0} & \val{37.5}{0.0} & \val{43.4}{1.8} & \val{50.8}{0.0} & \val{39.4}{0.0} & \val{78.0}{0.0} & 50.6 & 7.00  \\ 

     & ICL & \val{60.7}{16.7} & \val{55.2}{4.7} & \val{33.3}{13.1} & \val{46.8}{6.5} & \val{50.4}{0.6} & \val{63.8}{0.9} & \val{88.7}{0.5} & 57.0 & 5.43  \\ 
     
    \bottomrule 
    \end{tabular}    
    

\end{table}



==> tables/on_device_in_general.tex <==
\begin{table}[!htbp]
     \setlength{\tabcolsep}{3.8pt}
     \renewcommand{\arraystretch}{1.15} % Default value: 1
     \fontsize{8pt}{8pt}\selectfont
    \centering

    \vspace{-1.3em}
    \caption{Performance of sensitive sparse ZO fine-tuning with 99.9\% sparsity. In the first column, ``Q'' means the full model is quantized with 4-bit quantization method (SqueezeLLM~\citep{kim2023squeezellm}), and ``ZO'' means the model is finetuned with ZO-SGD optimizer. We follow the exact LoRA and Prefix-Tuning parameters shown in \citet{malladi2023fine}.
    For each cell, we use the same hyperparameters and repeat it with 3 random seeds. We report the average and standard deviation of test set accuracy in the format of \textbf{\val{\text{mean}}{\text{std}}}. In last 2 columns, ``Acc'' means the average test set accuracy and ``Rank'' means the average rank among all methods across tasks. }  \label{tab:main-results}

    \begin{subtable}[!ht]{\textwidth}
    \caption{\textbf{LlaMA2-7B}}
    \vspace{-0.5em}

    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l |c | ccccccc | ccr}
    \toprule    
     & \textbf{Methods} & SST-2 & RTE & CB & BoolQ & WSC & WiC & COPA & \textbf{Acc} & \textbf{Rank} \\ \hline
    
    \midrule

     Q, ZO & \textbf{Sensitive (C4, static)} & \val{\textbf{94.7}}{0.4} & \val{\textbf{74.7}}{1.2} & \val{\textbf{66.7}}{2.2} & \val{\textbf{83.0}}{0.5} & \val{57.4}{3.9} & \val{\textbf{65.2}}{0.9} & \val{85.0}{2.2} & \textbf{75.2} & \textbf{2.43} \\ 

     & LoRA & \val{93.8}{0.6} & \val{64.7}{1.1} & \val{64.9}{4.7} & \val{79.7}{1.1} & \val{\textbf{61.5}}{2.1} & \val{59.8}{0.1} & \val{\textbf{85.7}}{0.5} & 72.9 & 4.29 \\ 

     & Prefix & \val{80.5}{4.3} & \val{65.5}{1.2} & \val{63.1}{3.0} & \val{80.3}{0.2} & \val{54.5}{11.4} & \val{58.3}{1.3} & \val{82.0}{0.8} & 69.2 & 5.86 \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} & \val{\textbf{94.8}}{0.1} & \val{\textbf{73.6}}{0.9} & \val{\textbf{69.1}}{2.2} & \val{\textbf{83.5}}{0.8} & \val{57.4}{4.7} & \val{64.2}{1.1} & \val{\textbf{83.7}}{2.4} & \textbf{75.2} & \textbf{2.29} \\ 

     & Random (static) & \val{94.1}{0.3} & \val{68.0}{1.7} & \val{64.9}{3.4} & \val{77.0}{0.7} & \val{\textbf{59.6}}{3.6} & \val{\textbf{64.8}}{1.1} & \val{83.3}{1.7} & 73.1 & 4.14  \\ 

     & Full fine-tuning & \val{94.6}{0.5} & \val{73.3}{5.1} & \val{66.7}{0.8} & \val{81.9}{0.8} & \val{58.0}{4.3} & \val{61.9}{0.2} & \val{82.7}{1.7} & 74.2 & 3.57 \\ 

     \midrule

     & Zero-shot & \val{89.0}{0.0} & \val{57.8}{0.0} & \val{32.1}{0.0} & \val{69.9}{0.2} & \val{50.2}{0.0} & \val{36.5}{0.0} & \val{79.0}{0.0} & 59.2 & 7.29 \\ 


     & ICL & \val{94.8}{0.2} & \val{71.5}{4.3} & \val{72.6}{15.2} & \val{77.5}{4.6} & \val{53.2}{1.1} & \val{61.1}{4.3} & \val{87.0}{2.2} & 74.0 & 3.43 \\ 
     

    \bottomrule 
    \end{tabular*}
    
    \end{subtable}



    \vspace{-0.5em}
    \begin{subtable}[!ht]{\textwidth}
    \caption{\textbf{Mistral-7B}}
    \vspace{-0.5em}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l |c | ccccccc | ccr}

    \midrule

    Q, ZO & \textbf{Sensitive (C4, static)} & \val{\textbf{94.0}}{0.3} & \val{\textbf{74.2}}{2.7} & \val{\textbf{70.2}}{2.2} & \val{\textbf{75.1}}{2.4} & \val{59.6}{4.9} & \val{\textbf{61.2}}{0.9} & \val{\textbf{88.3}}{1.2} & \textbf{74.7} & \textbf{2.86} \\ 

     & LoRA & \val{\textbf{94.0}}{0.4} & \val{65.3}{1.3} & \val{64.9}{4.5} & \val{70.3}{3.7} & \val{\textbf{60.9}}{3.7} & \val{61.1}{0.4} & \val{\textbf{88.3}}{0.5} & 72.1 & 3.57 \\ 

     & Prefix & \val{86.9}{2.1} & \val{57.3}{1.4} & \val{63.7}{5.9} & \val{62.2}{0.9} & \val{60.3}{4.6} & \val{49.0}{0.3} & \val{81.3}{1.7} & 65.8 & 4.86 \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} & \val{\textbf{94.7}}{0.3} & \val{\textbf{77.1}}{0.9} & \val{\textbf{69.0}}{0.8} & \val{\textbf{78.4}}{2.2} & \val{\textbf{58.0}}{4.3} & \val{61.4}{0.2} & \val{\textbf{89.3}}{1.3} & \textbf{75.4} & \textbf{1.86} \\ 

     & Random (static) & \val{87.9}{1.9} & \val{50.2}{0.8} & \val{66.1}{4.4} & \val{60.6}{1.7} & \val{57.6}{1.4} & \val{57.3}{0.8} & \val{82.3}{1.7} & 66.0 & 5.29 \\ 

     & Full fine-tuning & \val{94.6}{0.1} & \val{74.6}{2.1} & \val{68.8}{6.2} & \val{76.6}{0.2} & \val{54.8}{6.2} & \val{\textbf{62.6}}{0.5} & \val{88.3}{0.5} & 74.3 & 2.86  \\ 

     \midrule

    & Zero-shot & \val{54.8}{0.0} & \val{50.5}{0.0} & \val{37.5}{0.0} & \val{43.4}{1.8} & \val{50.8}{0.0} & \val{39.4}{0.0} & \val{78.0}{0.0} & 50.6 & 7.00  \\ 

     & ICL & \val{60.7}{16.7} & \val{55.2}{4.7} & \val{33.3}{13.1} & \val{46.8}{6.5} & \val{50.4}{0.6} & \val{63.8}{0.9} & \val{88.7}{0.5} & 57.0 & 5.43  \\ 


    \bottomrule 
    \end{tabular*}   
    
    \end{subtable}


    \begin{subtable}[!ht]{\textwidth}
    \vspace{-0.5em}
    \caption{\textbf{OPT-6.7B}}
    \vspace{-0.5em}

    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l |c | ccccccc | ccr}

    \midrule

    Q, ZO & \textbf{Sensitive (C4, static)} & \val{\textbf{94.9}}{0.5} & \val{\textbf{72.8}}{3.6} & \val{\textbf{83.3}}{5.1} & \val{\textbf{73.1}}{0.9} & \val{\textbf{59.3}}{5.3} & \val{\textbf{60.9}}{0.4} & \val{\textbf{84.0}}{1.4} & \textbf{75.5} & \textbf{1.29} \\ 

     & LoRA & \val{94.2}{0.2} & \val{69.6}{1.6} & \val{69.0}{1.7} & \val{69.6}{2.0} & \val{57.1}{9.1} & \val{57.2}{0.8} & \val{83.0}{2.2} & 71.4 & 4.57 \\ 
     
     & Prefix & \val{93.3}{0.4} & \val{71.2}{1.0} & \val{72.0}{1.7} & \val{68.9}{2.8} & \val{62.5}{2.4} & \val{59.4}{0.5} & \val{80.0}{2.4} & 72.5 & 4.14 \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} & \val{\textbf{94.5}}{0.4} & \val{\textbf{75.5}}{1.4} & \val{\textbf{82.1}}{3.6} & \val{\textbf{72.5}}{0.8} & \val{\textbf{57.4}}{5.2} & \val{\textbf{60.6}}{1.4} & \val{\textbf{83.3}}{1.7} & \textbf{75.1} & \textbf{2.14} \\ 
     
     & Random (static) & \val{87.3}{2.0} & \val{68.4}{1.7} & \val{70.6}{6.3} & \val{66.0}{1.0} & \val{58.0}{7.0} & \val{56.4}{1.3} & \val{79.0}{0.8} & 69.4 & 5.71 \\ 

     & Full fine-tuning & \val{94.4}{0.3} & \val{72.7}{1.2} & \val{79.8}{3.0} & \val{72.1}{1.2} & \val{\textbf{57.4}}{4.6} & \val{60.2}{0.9} & \val{82.3}{2.6} & 74.1 & 3.29 \\ 

     \midrule

    & Zero-shot & \val{61.0}{0.0} & \val{60.7}{0.0} & \val{46.4}{0.0} & \val{55.7}{1.0} & \val{55.5}{0.0} & \val{36.5}{0.0} & \val{77.0}{0.0} & 56.1 & 7.71 \\ 
    % \cline{3-10}


     & ICL & \val{74.0}{14.6} & \val{65.8}{11.2} & \val{54.8}{5.9} & \val{67.9}{2.1} & \val{53.2}{1.7} & \val{41.0}{4.5} & \val{80.7}{2.9} & 62.5 & 6.57 \\ 
     





    \bottomrule 
    \end{tabular*}   

    \end{subtable}
\vspace{-2mm}
\end{table}

% 

==> tables/opt_6_7b.tex <==
\begin{table}[!ht]
     \setlength{\tabcolsep}{3.8pt}
     \renewcommand{\arraystretch}{1.25} % Default value: 1
     \fontsize{8pt}{8pt}\selectfont
    \centering
    
    \caption{Experiments on OPT-6.7B. }
    \label{tab:opt-6.7b}

    \begin{tabular}{l |c | ccccccc | ccr}
    \toprule    
     & \textbf{Methods} & SST-2 & RTE & CB & BoolQ & WSC & WiC & COPA & \textbf{Acc} & \textbf{Rank} \\ \hline
    
    \midrule

    Q, ZO & \textbf{Sensitive (C4, static)} & \val{\textbf{94.9}}{0.5} & \val{\textbf{72.8}}{3.6} & \val{\textbf{83.3}}{5.1} & \val{\textbf{73.1}}{0.9} & \val{\textbf{59.3}}{5.3} & \val{\textbf{60.9}}{0.4} & \val{\textbf{84.0}}{1.4} & \textbf{75.5} & \textbf{1.29} \\ 

     & LoRA & \val{94.2}{0.2} & \val{69.6}{1.6} & \val{69.0}{1.7} & \val{69.6}{2.0} & \val{57.1}{9.1} & \val{57.2}{0.8} & \val{83.0}{2.2} & 71.4 & 4.57 \\ 
     
     & Prefix & \val{93.3}{0.4} & \val{71.2}{1.0} & \val{72.0}{1.7} & \val{68.9}{2.8} & \val{62.5}{2.4} & \val{59.4}{0.5} & \val{80.0}{2.4} & 72.5 & 4.14 \\ 

    \midrule

    ZO & \textbf{Sensitive (task, static)} & \val{\textbf{94.5}}{0.4} & \val{\textbf{75.5}}{1.4} & \val{\textbf{82.1}}{3.6} & \val{\textbf{72.5}}{0.8} & \val{\textbf{57.4}}{5.2} & \val{\textbf{60.6}}{1.4} & \val{\textbf{83.3}}{1.7} & \textbf{75.1} & \textbf{2.14} \\ 
     
     & Random (static) & \val{87.3}{2.0} & \val{68.4}{1.7} & \val{70.6}{6.3} & \val{66.0}{1.0} & \val{58.0}{7.0} & \val{56.4}{1.3} & \val{78.3}{0.9} & 69.3 & 5.71 \\ 

     & Full fine-tuning & \val{94.4}{0.3} & \val{72.7}{1.2} & \val{79.8}{3.0} & \val{72.1}{1.2} & \val{\textbf{57.4}}{4.6} & \val{60.2}{0.9} & \val{82.3}{2.6} & 74.1 & 3.29 \\ 

     \midrule

    & Zero-shot & \val{61.0}{0.0} & \val{60.7}{0.0} & \val{46.4}{0.0} & \val{55.7}{1.0} & \val{55.5}{0.0} & \val{36.5}{0.0} & \val{77.0}{0.0} & 56.1 & 7.71 \\ 


     & ICL & \val{74.0}{14.6} & \val{65.8}{11.2} & \val{54.8}{5.9} & \val{67.9}{2.1} & \val{53.2}{1.7} & \val{41.0}{4.5} & \val{80.7}{2.9} & 62.5 & 6.57 \\ 
     


    \bottomrule 
    \end{tabular}    

\end{table}
